HALOGAS: Strong Constraints on the Neutral Gas Reservoir and Accretion Rate in Nearby Spiral Galaxies

Galaxies in the local Universe are thought to require ongoing replenishment of their gas reservoir in order to maintain the observed star formation rates. Cosmological simulations predict that such accretion can occur in both a dynamically hot and cold mode. However, until now observational evidence of the accretion required to match the observed star formation histories is lacking. This paper attempts to determine whether galaxies in the local Universe possess a significant reservoir of HI and what would be the accretion rates derived from such reservoirs. We search the vicinity of 22 nearby galaxies for isolated HI clouds or distinct streams in a systematic and automated manner. The HALOGAS observations represent one of the most sensitive and detailed HI surveys to date. These observations typically reach column density sensitivities of 10^19 cm^-2 over a 20 km/s width. We find 14 secure HI cloud candidates without an observed optical counterpart. These cloud candidates appear to be analogues to the most massive clouds detected around the Milky Way and M31. However, on average their numbers seem significantly reduced. We constrain upper limits for HI accretion in the local Universe. The average HI mass currently observed amounts to a rate of 0.05 Msun/yr with a stringent upper limit of 0.22 Msun/yr, confirming previous estimates. This is much lower than the average star formation rate in this sample. Our best estimate, based on GBT detection limits of several galaxies, suggests that another 0.04 Msun/yr could be accreted from undetected clouds and streams. These results show that in nearby galaxies HI is not being accreted at the same rate as stars are currently being formed. Our study can not exclude that other forms of gas accretion are at work. However, these observations also do not reveal extended neutral gas reservoirs around most nearby spiral galaxies.

==> Accretion_Clouds.tex <==
% This file contains the Accretion quantities of clouds info. 
\begin{table*}[ht!] 
\caption{Accretion rate estimates of the cloud candidates.} \label{table:accretion_clouds} 
\centering  
\begin{tabular}{c c c c c c c } 
\hline 
Host Galaxy & Source & v$_{esc}$&  $t_{\rm ff1}$ & $t_{\rm ff2}$ & \.M$_1$ & \.M$_2$  \\ 
        &  & \kms& $10^{7}$ yr &  $10^{7}$ yr & \msun yr$^{-1}$& \msun yr$^{-1}$ \\ 
\hline 
NGC\,0925  & 2 &      216.4 &         16 &          6 &      0.007 &      0.016  \\ 
NGC\,1003  & 2 &      300.7 &          6 &          3 &       0.04 &       0.08  \\ 
NGC\,4258  & 3 &      353.7 &         10 &          2 &       0.01 &       0.04  \\ 
NGC\,4258  & 8 &      301.1 &         17 &          7 &       0.01 &       0.03  \\ 
NGC\,4274  & 9 &      146.3 &        113 &        107 &      0.005 &      0.006  \\ 
NGC\,4274  & 10 &      159.5 &         87 &         81 &      0.008 &      0.008  \\ 
NGC\,4274  & 11 &      342.4 &          8 &          5 &       0.11 &       0.18  \\ 
NGC\,4414  & 2 &      341.9 &         19 &          8 &       0.02 &       0.05  \\ 
NGC\,4565  & 3 &      434.6 &          8 &          4 &       0.02 &       0.04  \\ 
NGC\,4565  & 6 &      392.3 &         11 &         10 &      0.007 &      0.009  \\ 
NGC\,4565  & 7 &      393.6 &         11 &          6 &       0.02 &       0.03  \\ 
NGC\,4565  & 8 &      207.9 &         79 &         64 &       0.01 &       0.02  \\ 
NGC\,5055  & 2 &      379.7 &         14 &          5 &       0.05 &       0.14  \\ 
NGC\,5585  & 1 &       82.8 &        115 &         91 &      0.001 &      0.001  \\ 
\hline 
\end{tabular} 
	\tablefoot{ The difference between \.M$_1$ and \.M$_2$ can be considered as an indication of the uncertainty on these upper limits.
} 
\end{table*} 


==> Accretion_Companions.tex <==
% This file contains the Accretion quantities of companions info. 
\begin{table*}[ht!] 
\caption{Accretion rate estimates of the companion candidates.} \label{table:accretion_companions} 
\centering  
\begin{tabular}{c c c c c c c } 
\hline 
Host Galaxy & Source & v$_{esc}$&  $t_{\rm ff1}$ & $ t_{\rm ff2}$ & \.M$_1$ & \.M$_2$  \\ 
        &  & \kms& $10^{7}$ yr &  $10^{7}$ yr & \msun yr$^{-1}$& \msun yr$^{-1}$ \\ 
\hline 
NGC\,0925  & 2 &      216.4 &         16 &          6 &      0.007 &      0.016  \\ 
NGC\,0925  & 4 &      132.9 &         69 &         51 &       0.02 &       0.02  \\ 
NGC\,1003  & 2 &      300.7 &          6 &          3 &       0.04 &       0.08  \\ 
NGC\,2541  & 1 &       79.1 &        227 &        198 &       0.02 &       0.02  \\ 
NGC\,3198  & 2 &      140.6 &        149 &        137 &       0.18 &       0.19  \\ 
NGC\,4258  & 3 &      353.7 &         10 &          2 &       0.01 &       0.04  \\ 
NGC\,4258  & 4 &      240.3 &         33 &         24 &       0.13 &       0.18  \\ 
NGC\,4258  & 6 &      329.7 &         13 &          8 &       0.28 &       0.45  \\ 
NGC\,4258  & 8 &      301.1 &         17 &          7 &       0.01 &       0.03  \\ 
NGC\,4258  & 10 &      501.2 &          3 &          1 &       0.02 &       0.06  \\ 
NGC\,4274  & 9 &      146.3 &        113 &        107 &      0.005 &      0.006  \\ 
NGC\,4274  & 10 &      159.5 &         87 &         81 &      0.008 &      0.008  \\ 
NGC\,4274  & 11 &      342.4 &          8 &          5 &       0.11 &       0.18  \\ 
NGC\,4414  & 2 &      341.9 &         19 &          8 &       0.02 &       0.05  \\ 
NGC\,4565  & 1 &      389.1 &         12 &         10 &       0.02 &       0.03  \\ 
NGC\,4565  & 3 &      434.6 &          8 &          4 &       0.02 &       0.04  \\ 
NGC\,4565  & 4 &      335.0 &         18 &         16 &       0.92 &       1.03  \\ 
NGC\,4565  & 5 &      529.1 &          4 &          3 &       0.82 &       1.30  \\ 
NGC\,4565  & 6 &      392.3 &         11 &         10 &      0.007 &      0.009  \\ 
NGC\,4565  & 7 &      393.6 &         11 &          6 &       0.02 &       0.03  \\ 
NGC\,5055  & 2 &      379.7 &         14 &          5 &       0.05 &       0.14  \\ 
NGC\,5055  & 4 &      300.1 &         29 &         19 &       0.29 &       0.44  \\ 
\hline 
\end{tabular} 
	\tablefoot{The difference between \.M$_1$ and \.M$_2$ can be considered as an indication of the uncertainty on these upper limits.
} 
\end{table*} 


==> Accretion_Upper_Final.tex <==
% This file contains the Accretion quantities for the Upper limit. 
\begin{table*}[ht!] 
\caption{Accretion rate upper limits for the sample.} \label{table:accretion_upper} 
\centering  
\begin{tabular}{c c c c c c } 
\hline 
Host Galaxy & Detect. Limit & Detect. Limit& ${\rm \dot{M}}_{f=0.1}$ & ${\rm \dot{M}}_{f=3\times10^{-5}}$ &  ${\rm \dot{M}}_{\rm GBT}$ \\ 
        &  mJy \kms & 10$^5$\msun & \msun yr$^{-1}$ & \msun yr$^{-1}$ & \msun yr$^{-1}$\\ 
\hline 
NGC0925    &       24.2 &        4.7 &       8.07 &      0.002 &      0.034 \\ 
NGC0949    &       23.5 &        7.1 &       1.23 &      0.000 &      0.010 \\ 
NGC1003    &       24.4 &        7.8 &       5.24 &      0.002 &      0.014 \\ 
NGC2541    &       26.9 &        9.1 &      12.89 &      0.004 &      0.023 \\ 
NGC3198    &       22.1 &       11.0 &      14.53 &      0.004 &      0.037 \\ 
NGC4062    &       26.8 &       18.1 &       2.36 &      0.001 &      0.034 \\ 
NGC4244    &       21.4 &        1.0 &       9.20 &      0.003 &      0.024 \\ 
NGC4258    &       29.6 &        4.0 &      38.66 &      0.012 &      0.074 \\ 
NGC4274    &       22.1 &       19.6 &       3.81 &      0.001 &      0.106 \\ 
NGC4414    &       24.8 &       18.5 &       2.06 &      0.001 &      0.021 \\ 
NGC4448    &       23.4 &        5.2 &       0.62 &      0.000 &      0.037 \\ 
NGC4559    &       23.2 &        3.4 &       4.13 &      0.001 &      0.035 \\ 
NGC4565    &       22.5 &        6.2 &       9.14 &      0.003 &      0.122 \\ 
NGC5023    &       27.5 &        2.8 &       4.64 &      0.001 &      0.017 \\ 
NGC5055    &       25.0 &        4.3 &      17.98 &      0.005 &      0.032 \\ 
NGC5229    &       23.8 &        1.5 &       0.98 &      0.000 &      0.004 \\ 
NGC5585    &       23.5 &        4.2 &       6.15 &      0.002 &      0.009 \\ 
UGC2082    &       27.0 &       12.6 &       2.14 &      0.001 &      0.025 \\ 
UGC4278    &       23.4 &       10.2 &       3.54 &      0.001 &      0.021 \\ 
UGC7774    &       27.5 &       38.6 &       3.49 &      0.001 &      0.019 \\ 
\hline 
\end{tabular} 
\end{table*} 


==> Clouds_Table.tex <==
% This file contains the final cloud sources table 
\onecolumn
\begin{landscape} 
\begin{table}\label{table:clouds} 
\caption{\sofia\ detected Cloud Candidates.} \label{table:cloud} 
\centering 
\begin{tabular}{lllllllllllll}
\hline 
Galaxy & ID & RA & Dec & Class  & S$_{p}$ & $F_{i}$  & $F_{i}$,pbcorr & W20  & Vel. & Dist. to target & Flag \\ 
  &   &  [hms] & [dms] & &   [mJy  bm$^{-1}$] & [Jy \kms] & [Jy \kms] & [\kms] & [\kms] & [kpc] &  \\ 
   (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)   \\  
\hline 
NGC\,0925  & 2          & 2h27m5.62s   & 33d43m13.73s & CC     & 0.871      & 0.048     & 0.056      & 45.1       & 579.1      & 22.6       & 2      \\ 
NGC\,1003  & 2          & 2h39m12.94s  & 40d55m51.93s & CC     & 0.893      & 0.086     & 0.088      & 36.3       & 593.9      & 12.3       & 1      \\ 
NGC\,4258  & 3          & 12h19m2.16s  & 47d6m52.02s  & CC     & 0.830      & 0.067     & 0.088      & 41.5       & 252.9      & 24.5       & 1      \\ 
NGC\,4258  & 8          & 12h18m34.75s & 47d32m46.60s & CC     & 1.174      & 0.088     & 0.141      & 42.0       & 570.7      & 33.8       & 2      \\ 
NGC\,4274  & 9          & 12h20m18.55s & 29d18m48.96s & CC     & 1.082      & 0.032     & 0.069      & 30.3       & 791.7      & 108.4      & 1      \\ 
NGC\,4274  & 10         & 12h20m18.47s & 29d22m2.91s  & CC     & 0.962      & 0.045     & 0.077      & 32.9       & 979.4      & 91.3       & 1      \\ 
NGC\,4274  & 11         & 12h20m0.86s  & 29d34m26.72s & CC     & 1.224      & 0.110     & 0.112      & 42.2       & 998.7      & 19.8       & 1      \\ 
NGC\,4414  & 2          & 12h26m26.93s & 31d21m20.80s & CC     & 0.888      & 0.045     & 0.051      & 36.0       & 622.0      & 42.8       & 1      \\ 
NGC\,4565  & 3          & 12h36m49.28s & 25d55m49.89s & CC     & 0.799      & 0.058     & 0.065      & 50.4       & 1017.6     & 24.6       & 2      \\ 
NGC\,4565  & 6          & 12h35m39.69s & 25d55m58.35s & CC     & 1.092      & 0.025     & 0.031      & 25.9       & 1327.0     & 30.2       & 1      \\ 
NGC\,4565  & 7          & 12h35m59.96s & 26d8m16.66s  & CC     & 0.785      & 0.057     & 0.070      & 37.3       & 1381.8     & 30.0       & 2      \\ 
NGC\,4565  & 8          & 12h38m11.61s & 25d36m44.94s & CC     & 0.991      & 0.030     & 0.411      & 98.2       & 1576.6     & 107.5      & 2      \\ 
NGC\,5055  & 2          & 13h16m59.56s & 42d6m39.26s  & CC     & 0.981      & 0.309     & 0.462      & 48.6       & 534.6      & 36.3       & 2      \\ 
NGC\,5585  & 1          & 14h21m24.29s & 57d4m47.70s  & CC     & 0.916      & 0.020     & 0.076      & 63.1       & 111.0      & 62.0       & 2      \\ 
\hline 
\end{tabular} 
\end{table} 
\end{landscape}
\twocolumn 


==> Figures_App_New/Cloud_images.tex <==
%This file contains all the images for the cloud sources 
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n0925_image_src_2.pdf} 
\caption{From left to right: Optical image overlaid with contours of the \hi moment 0 (intensity) map , moment 1 (velocity ) map,  PV-Diagram along major axis and line profile for source no. 2 in the cube of NGC\,0925. Contours for moment 0 are: 6.8, 27.2, 54.4$\times 10^{18} {\rm cm}^{-2}$  overlaid on our HALOSTARS $R$-band image. These are corrected with the same factor as the integrated flux in the various tables to account for the primary beam response. The blue ellipse indicates the \sofia\ fitted ellipse. Contours for the velocity field start at 560.36 km\,s$^{-1}$ and increase with 5.00 km\,s$^{-1}$. The PV-diagram is extracted at a PA of 206$^{\circ}$ with contours at -3, -1.5, 1.5, 3 $\sigma$, with $\sigma=0.160$ mJy beam$^{-1}$.} 
\label{fig:n0925_image_src_2.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n1003_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 2 in the cube of NGC\,1003. Contours for moment 0 are: 7.7, 31.0, 62.0$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 571.56 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 123$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.182$ mJy beam$^{-1}$.} 
\label{fig:n1003_image_src_2.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4258_image_src_3.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 3 in the cube of NGC\,4258. Contours for moment 0 are: 1.2, 5.0$\times 10^{19} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 238.00 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 148$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.215$ mJy beam$^{-1}$.} 
\label{fig:n4258_image_src_3.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4258_image_src_8.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 8 in the cube of NGC\,4258. Contours for moment 0 are: 1.6, 6.5$\times 10^{19} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 555.24 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 349$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.227$ mJy beam$^{-1}$.} 
\label{fig:n4258_image_src_8.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4274_image_src_9.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 9 in the cube of NGC\,4274. Contours for moment 0 are: 1.1, 4.5, 9.0$\times 10^{19} {\rm cm}^{-2}$. Contours for the velocity field start at 781.04 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 186$^{\circ}$ with contours at -1.5, 1.5 $\sigma$, with $\sigma=0.173$ mJy beam$^{-1}$.} 
\label{fig:n4274_image_src_9.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4274_image_src_10.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 10 in the cube of NGC\,4274. Contours for moment 0 are: 8.3, 33.1, 66.3$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 962.32 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 206$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.161$ mJy beam$^{-1}$.} 
\label{fig:n4274_image_src_10.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4274_image_src_11.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 11 in the cube of NGC\,4274. Contours for moment 0 are: 5.3, 21.2, 42.5, 63.7$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 978.80 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 71$^{\circ}$ with contours at -1.5, 1.5, 3, 6 $\sigma$, with $\sigma=0.172$ mJy beam$^{-1}$.} 
\label{fig:n4274_image_src_11.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4414_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 2 in the cube of NGC\,4414. Contours for moment 0 are: 6.1, 24.2$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 609.16 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 139$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.189$ mJy beam$^{-1}$.} 
\label{fig:n4414_image_src_2.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4565_image_src_3.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 3 in the cube of NGC\,4565. Contours for moment 0 are: 5.8, 23.1, 46.2$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 996.40 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 13$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.170$ mJy beam$^{-1}$.} 
\label{fig:n4565_image_src_3.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4565_image_src_6.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 6 in the cube of NGC\,4565. Contours for moment 0 are: 5.0, 19.9, 39.8$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 1317.76 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 341$^{\circ}$ with contours at -1.5, 1.5, 3, 6 $\sigma$, with $\sigma=0.156$ mJy beam$^{-1}$.} 
\label{fig:n4565_image_src_6.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4565_image_src_7.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 7 in the cube of NGC\,4565. Contours for moment 0 are: 7.3, 29.0$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 1363.08 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 5$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.211$ mJy beam$^{-1}$.} 
\label{fig:n4565_image_src_7.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n4565_image_src_8.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 8 in the cube of NGC\,4565. Contours for moment 0 are: 9.6, 38.5, 77.0, 153.9$\times 10^{19} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the HALOSTARS field. Contours for the velocity field start at 1527.88 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 186$^{\circ}$ with contours at -1.5, 1.5, 3 $\sigma$, with $\sigma=0.193$ mJy beam$^{-1}$.} 
\label{fig:n4565_image_src_8.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n5055_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 2 in the cube of NGC\,5055. Contours for moment 0 are: 1.2, 4.8, 9.6, 14.4$\times 10^{19} {\rm cm}^{-2}$. Contours for the velocity field start at 511.92 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 209$^{\circ}$ with contours at -3, -1.5, 1.5, 3 $\sigma$, with $\sigma=0.187$ mJy beam$^{-1}$.} 
\label{fig:n5055_image_src_2.pdf}
\end{figure*}
\begin{figure*} 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/n5585_image_src_1.pdf} 
\caption{ As \ref{fig:n0925_image_src_2.pdf} but for source no. 1 in the cube of NGC\,5585. Contours for moment 0 are: 6.1, 24.2, 48.4$\times 10^{19} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 78.12 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. The PV-diagram is extracted at a PA of 135$^{\circ}$ with contours at , 1.5, 3, 6 $\sigma$, with $\sigma=0.274$ mJy beam$^{-1}$.} 
\label{fig:n5585_image_src_1.pdf}
\end{figure*}


==> Figures_App_New/Ind_sources_images.tex <==
%This file contains all the images addition for all real sources 
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n0925_image_src_4.pdf} 
\caption{Moment maps for source no. 4 in the cube of NGC\,0925. Contours for moment 0 are: 1.9, 7.6, 15.2, 30.4, 45.6$\times 10^{19} {\rm cm}^{-2}$  overlaid on our HALOSTARS $R$-band image. These are corrected with the same factor as the integrated flux in the various tables to account for the primary beam response. The blue ellipse indicates the SoFiA fitted ellipse. Contours for the velocity field start at 622.16 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$.} 
\label{fig:n0925_image_src_4.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n2541_image_src_1.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 1 in the cube of NGC\,2541. Contours for moment 0 are: 1.4, 5.5, 11.0, 16.5$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the HALOSTARS field. Contours for the velocity field start at 494.44 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as WISEA\,J081239.49+483645.3.} 
\label{fig:n2541_image_src_1.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n3198_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 2 in the cube of NGC\,3198. Contours for moment 0 are: 1.1, 4.2, 8.5, 16.9, 25.4, 33.8$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the HALOSTARS field. Contours for the velocity field start at 543.76 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as VV\,834\,NED02.} 
\label{fig:n3198_image_src_2.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4258_image_src_4.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 4 in the cube of NGC\,4258. Contours for moment 0 are: 3.4, 13.7$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 349.24 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$.} 
\label{fig:n4258_image_src_4.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4258_image_src_6.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 6 in the cube of NGC\,4258. Contours for moment 0 are: 1.3, 5.3, 10.5$\times 10^{20} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 423.40 km\,s$^{-1}$ and increase with 5.77 km s$^{-1}$. This source is identified as NGC\,4248.} 
\label{fig:n4258_image_src_6.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4258_image_src_9.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 9 in the cube of NGC\,4258. Contours for moment 0 are: 2.2, 8.8, 17.6, 35.2, 52.8$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 823.04 km\,s$^{-1}$ and increase with 19.98 km s$^{-1}$.} 
\label{fig:n4258_image_src_9.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4258_image_src_10.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 10 in the cube of NGC\,4258. Contours for moment 0 are: 1.2, 4.8, 9.6$\times 10^{19} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 798.32 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$.} 
\label{fig:n4258_image_src_10.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4258_image_src_11.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 11 in the cube of NGC\,4258. Contours for moment 0 are: 1.1, 4.3, 8.6$\times 10^{19} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 930.16 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$.} 
\label{fig:n4258_image_src_11.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4274_image_src_1.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 1 in the cube of NGC\,4274. Contours for moment 0 are: 1.6, 6.6, 13.1, 19.7$\times 10^{19} {\rm cm}^{-2}$. Contours for the velocity field start at 377.28 km\,s$^{-1}$ and increase with 23.90 km s$^{-1}$.} 
\label{fig:n4274_image_src_1.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4274_image_src_6.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 6 in the cube of NGC\,4274. Contours for moment 0 are: 1.5, 6.2, 12.4, 24.7, 37.1$\times 10^{19} {\rm cm}^{-2}$. Contours for the velocity field start at 575.04 km\,s$^{-1}$ and increase with 6.59 km s$^{-1}$. This source is identified as NGC\,4286.} 
\label{fig:n4274_image_src_6.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4414_image_src_7.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 7 in the cube of NGC\,4414. Contours for moment 0 are: 1.2, 4.8, 9.6, 19.2, 28.8$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the HALOSTARS field. Contours for the velocity field start at 1136.52 km\,s$^{-1}$ and increase with 10.92 km s$^{-1}$. This source is identified as NGC\,4359.} 
\label{fig:n4414_image_src_7.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4448_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 2 in the cube of NGC\,4448. Contours for moment 0 are: 4.0, 15.9, 31.8, 63.6$\times 10^{19} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image. Contours for the velocity field start at 1186.52 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as IC\,3334.} 
\label{fig:n4448_image_src_2.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4559_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 2 in the cube of NGC\,4559. Contours for moment 0 are: 2.4, 9.4, 18.9, 37.7, 56.6$\times 10^{19} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 1172.48 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as WISEA\,J123521.10+273342.9.} 
\label{fig:n4559_image_src_2.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4565_image_src_1.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 1 in the cube of NGC\,4565. Contours for moment 0 are: 5.9, 23.6, 47.2, 94.3$\times 10^{18} {\rm cm}^{-2}$. Contours for the velocity field start at 839.84 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$.} 
\label{fig:n4565_image_src_1.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4565_image_src_4.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 4 in the cube of NGC\,4565. Contours for moment 0 are: 6.7, 26.8, 53.6, 107.1, 160.7$\times 10^{19} {\rm cm}^{-2}$. Contours for the velocity field start at 1260.08 km\,s$^{-1}$ and increase with 8.45 km s$^{-1}$. This source is identified as NGC\,4562.} 
\label{fig:n4565_image_src_4.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4565_image_src_5.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 5 in the cube of NGC\,4565. Contours for moment 0 are: 5.4, 21.6, 43.3$\times 10^{19} {\rm cm}^{-2}$. Contours for the velocity field start at 1223.00 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as IC\,3571.} 
\label{fig:n4565_image_src_5.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4631_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 2 in the cube of NGC\,4631. Contours for moment 0 are: 7.1, 28.6, 57.2$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 514.72 km\,s$^{-1}$ and increase with 12.57 km s$^{-1}$. This source is identified as NGC\,4656.} 
\label{fig:n4631_image_src_2.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4631_image_src_6.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 6 in the cube of NGC\,4631. Contours for moment 0 are: 1.4, 5.4$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 646.56 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as SDSS\,J124146.99+325124.8.} 
\label{fig:n4631_image_src_6.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4631_image_src_9.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 9 in the cube of NGC\,4631. Contours for moment 0 are: 2.9, 11.5$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image as it is outside the KPNO field. Contours for the velocity field start at 712.48 km\,s$^{-1}$ and increase with 5.56 km s$^{-1}$. This source is identified as SDSS\,J124010.08+323930.4.} 
\label{fig:n4631_image_src_9.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4631_image_src_10.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 10 in the cube of NGC\,4631. Contours for moment 0 are: 10.0, 40.0, 79.9$\times 10^{19} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 852.56 km\,s$^{-1}$ and increase with 5.77 km s$^{-1}$. This source is identified as MCG\,+06-28-022.} 
\label{fig:n4631_image_src_10.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n4631_image_src_11.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 11 in the cube of NGC\,4631. Contours for moment 0 are: 7.3, 29.1, 58.2, 116.3$\times 10^{18} {\rm cm}^{-2}$ but overlaid on our KPNO $R$-band image. Contours for the velocity field start at 889.64 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$.} 
\label{fig:n4631_image_src_11.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n5055_image_src_4.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 4 in the cube of NGC\,5055. Contours for moment 0 are: 3.2, 12.9, 25.9$\times 10^{20} {\rm cm}^{-2}$. Contours for the velocity field start at 549.00 km\,s$^{-1}$ and increase with 7.42 km s$^{-1}$. This source is identified as UGC\,8313.} 
\label{fig:n5055_image_src_4.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/n5055_image_src_6.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 6 in the cube of NGC\,5055. Contours for moment 0 are: 1.3, 5.3, 10.7$\times 10^{20} {\rm cm}^{-2}$. Contours for the velocity field start at 1187.60 km\,s$^{-1}$ and increase with 7.21 km s$^{-1}$. This source is identified as UGC\,8365.} 
\label{fig:n5055_image_src_6.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/u4278_image_src_4.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 4 in the cube of UGC\,4278. Contours for moment 0 are: 1.3, 5.1, 10.2$\times 10^{20} {\rm cm}^{-2}$. Contours for the velocity field start at 349.88 km\,s$^{-1}$ and increase with 9.27 km s$^{-1}$. This source is identified as NGC\,2537.} 
\label{fig:u4278_image_src_4.pdf}
\end{figure}
\begin{figure} 
\centering 
\includegraphics[width = 8 cm]{Figures_App_New/u7774_image_src_2.pdf} 
\caption{ As \ref{fig:n0925_image_src_4.pdf} but for source no. 2 in the cube of UGC\,7774. Contours for moment 0 are: 2.2, 8.9, 17.8$\times 10^{20} {\rm cm}^{-2}$ but overlaid on a DDS 2 $R$-band image. Contours for the velocity field start at 632.24 km\,s$^{-1}$ and increase with 5.00 km s$^{-1}$. This source is identified as MCG\,+07-26-024.} 
\label{fig:u7774_image_src_2.pdf}
\end{figure}


==> Figures_App_New/Overview_images.tex <==
%This file contains all the Overview images 
\subsubsection{NGC 0925} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n0925.pdf} 
\caption{HALOSTARS image for the NGC\,0925 field overlaid with contours from the detected sources. Contour colours correspond to the systemic velocity of each source as determined by \sofia\ and indicated by the colorbar on the right. Contour levels vary per source and are listed in the captions of the individual images. The contours for the target correspond to 5.1, 20.5, 40.9, 81.8, 122.7, 162.3$\times 10^{19} {\rm cm}^{-2}$. The blue solid ellipse indicates the nominal virial radius (which can fall outside the field of view) and the dashed ellipse the FWHM of the WSRT primary beam. Labels indicate source number and class as listed in Tables \ref{table:accretion_clouds} and \ref{table:detec}. Blue crosses indicate galaxies spectroscopically confirmed to be in the velocity range of the cube.} 
\label{fig:Overview_n0925.pdf}
\end{figure*}
NGC\,925 is a spiral galaxy with an extended gas distribution and a XUV disk. Besides the target we find two more \hi\ sources. One detection (source 2) is found relatively close to the target galaxy and could be part of the extended low surface brightness disk. The projected distance to the center of the target galaxy  is $\sim$ 23 kpc  and its systemic velocity only differs by 30 \kms\ from NGC\,925. We could find no optical counterpart and hence it is classified as a cloud candidate. Technically the cloud is counter rotating. However, it is very close to the kinematic minor axis of the galaxy making the kinematical assessment difficult.\\
\indent The other detection (source 4) is separated from the target galaxy. It has an UV counterpart, as stated in \cite{KMK2013}, and also in our deep $R$-band image an optical counterpart can be seen (See Figure \ref{fig:n0925_image_src_4.pdf}). Its systemic velocity deviates about 90 \kms  from  NGC\,925  and it is at a projected distance of $\sim$ 62 kpc from the center of NGC\,925 and is co-rotating with its disk. 
\subsubsection{NGC 1003} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n1003.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,1003 field.} 
\label{fig:Overview_n1003.pdf}
\end{figure*}
This is an edge-on galaxy of which the \hi\ disk extends far beyond the visible optical disk. In the outer parts of the disk there are hints of warping and several clouds, considered to be HVC analogues, can be seen around the main disk \citep{Heald2011b}. These clouds are all detected however only one of them is separated from the emission in the disk (see section \ref{implicatcold} on how this affects our results).\\
\indent Even though this counter rotating  source is separated by more than a FWHM from the mask encompassing the emission of NGC\,1003, it is still close to the disk. The HALOSTARS image (Figure \ref{fig:n1003_image_src_2.pdf}) does not show an optical counterpart at its location, but the field is crowded with foreground stars making identification of low level optical emission difficult. 
\subsubsection{NGC 2541} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n2541.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,2541 field.} 
\label{fig:Overview_n2541.pdf}
\end{figure*}
A companion is found at a projected distance of 120 kpc with a velocity difference of only $\sim 40$ \kms (See Figure \ref{fig:n2541_image_src_1.pdf}). Even though the galaxy is warped, it appears rather regular and undisturbed. The detected companion is on the edge of the cube and hence its detection is too faint in \HI\ to provide any meaningful analysis about its structure or kinematics. 
\subsubsection{NGC 3198} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n3198.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,3198 field.} 
\label{fig:Overview_n3198.pdf}
\end{figure*}
This galaxy is extensively investigated for its halo properties in \cite{Gentile2013}.  It is a rather regular galaxy  where we detect a single companion galaxy at a projected distance $\sim$ 140 kpc. The systemic velocity of this companion is aligned with the rotation of NGC\,3198's disk. 
\subsubsection{NGC 4258} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4258.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4258 field overlaid on a KPNO $R$-band image.} 
\label{fig:Overview_n4258.pdf}
\end{figure*}
The field of NGC\,4258 is a rich field with several detections. The galaxy has four smaller companions which makes past or ongoing weak interaction very likely.  Besides the four companions the galaxy has several tails that run off from the main disk. These typically end in fragmented clouds. Sometimes these are connected to the disk, and merged with the galaxy in our source finding (see Figure \ref{fig:Overview_n4258.pdf} in the SE). In other instances, as in the case of our sources 3 and 8, these are distinct enough to be counted as individual detections. However, they all appear connected to the disk in some shape or form. As such it is impossible to tell whether they are infalling or being tidally stripped from the galaxy. All these detections follow the general rotation of the disk. Sources 9 and 11 are far beyond the velocity range of the disk however. \\
\indent For source 10 we could not spectroscopically confirm an optical counterpart however  our KPNO $R$ band image \ref{fig:n4258_image_src_10.pdf} shows a smudge of light. Hence it is classified as a companion. This source occurs close to the minor axis of the host and has a systemic velocity $\sim 75$ \kms, higher than the highest velocity in the disk of NGC\,4258, technically this means it is counter rotating. 
\subsubsection{NGC 4274}\label{ind:4274} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4274.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4274 field.} 
\label{fig:Overview_n4274.pdf}
\end{figure*}
NGC\,4274 is another rich field with at least three companion galaxies, NGC\,4286, NGC\,4283 and NGC\,4278. All  are about 90\,kpc to the south of the target and much closer to each other than to NGC\,4274. Their systemic velocities and locations are aligned with the rotation in the disk of NGC\,4274.  The \HI\ in NGC\,4278 is sporadic and fragmented. However, this appears to be more an effect of sensitivity than the actual distribution. Some \HI\ is detected toward NGC\,4283 but it appears to be part of foreground emission coming from NGC\,4278.\\
\indent We find three cloud candidates in this field. Two (Source 9 and 10) are closer to the system of companion galaxies and are most likely tidal debris of interactions between these galaxies. Source 10 would be counter rotating when compared to the disk of NGC\,4274 but is co-rotating with the companion galaxies and source 9 co-rotating with NGC\,4274.\\
\indent Source 11 is  close to NGC\,4274, extended and has a hint of rotation. Unfortunately the spatial resolution of the HALOGAS observations is not sufficient to confirm this rotation. Even in deep-follow up observations there appears to be no optical counterpart and hence we refer to this object as {\it'Dark galaxy candidate'}. If truly a galaxy, possibly with an undetected optical counterpart, it would be a companion instead of a cloud. This cloud candidate is counter-rotating from the perspective of NGC\,4274's disk.
\subsubsection{NGC 4414} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4414.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4414 field.} 
\label{fig:Overview_n4414.pdf}
\end{figure*}
The single cloud candidate detected in this cube appears at the end of a tail of the target galaxy and is co-rotating. In a galaxy of such low inclination this is likely material falling into the disk and not ejected from it as most of the ejection mechanisms work in a vertical direction compared to the disk orientation. Besides the detected cloud candidate, the galaxy also displays a significant extension in \hi\ to the North-West. In our source finding this has merged with the main disk. NGC\,4414 is the galaxy with the highest SFR in the sample and the HALOGAS data are previously described in \cite{deBlok2014}.\\
\indent Besides the target and cloud candidate, we also detect NGC\,4359. This galaxy is significantly removed from the target and its systemic velocity is not in alignment with the rotation of NGC\,4414's disk. 
\subsubsection{NGC 4448} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4448.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4448 field overlaid on a DSS 2 $R$-band image.} 
\label{fig:Overview_n4448.pdf}
\end{figure*}
NGC\,4448 is an isolated, regularly rotating galaxy seen at a high inclination. The \hi\ distribution in the galaxy appears to be rather compact despite having an average line width (see Table \ref{table:hosts}). The optical disk extends beyond the \hi\ disk which gives the impression of the gas in the outer regions being stripped.\\
\indent The galaxy IC\,3334 is also detected in the data cube albeit with a significantly higher systemic velocity. 
\subsubsection{NGC 4559} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4559.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4559 field overlaid on a KPNO $R$-band image.} 
\label{fig:Overview_n4559.pdf}
\end{figure*}
The HALOGAS data for NGC\,4559 are presented and discussed in detail in \cite{Vargas2017}. This is a moderately inclined galaxy without obvious peculiarities. We detect a single companion at a projected distance of 65 kpc. The companion shows no regular velocity structure and the \hi\ appears more extended than the optical from the WISE images. The difference in systemic velocity between this companion and NGC\,4559 is more than 400 \kms. 
\subsubsection{NGC 4565} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4565.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4565 field.} 
\label{fig:Overview_n4565.pdf}
\end{figure*}
NGC\,4565 is a disturbed galaxy with three companions. We find two anomalous gas clouds in this system that are close to the galaxy and we classify them as cloud candidates. Additionally we find another two cloud candidates in this data cube as well. All companions and cloud candidates are co-rotating with the disk of the galaxy except for source 8 which is furthest removed in velocity as well as projected distance.\\
\indent Tidal debris is a possible origin for the co-rotating cloud candidates, given the environment of interaction. This observation is extensively described in \cite{Zschaechner2012}. 
\subsubsection{NGC 4631} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n4631.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,4631 field overlaid on a KPNO $R$-band image.} 
\label{fig:Overview_n4631.pdf}
\end{figure*}
NGC\,4631 is a galaxy that is heavily interacting with its environment. This extended gas distribution was already seen in older observations \citep{Rand1994} and, as there is gas almost everywhere in the field of view, is complicated to "clean". Hence, significant side lobes of the dirty beam remain in the final data cube and we detect several artifacts.  Complicating matters even more, it appears that several real sources are situated on top of side lobe emission. They can be visually identified as they are so much brighter than the sidelobes but any velocity and flux measurements are highly unreliable. \\
\indent Besides the obvious companion NGC\,4656,  we detect  three companions which spatially coincide with the gas surrounding NGC\,4631 but are distinct in velocity space. Additionally, we detect a source that is further removed from the system. The latter (source 9) is the only companion which is not aligned with the rotational direction of the disk. \\
\indent As the galaxy is in an equal mass merger and due to the issues with the side lobes we exclude it from  the analysis presented in this paper. 
\subsubsection{NGC 5055} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n5055.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,5055 field.} 
\label{fig:Overview_n5055.pdf}
\end{figure*}
This is a large spiral galaxy. Besides the target we detect two companions, UGC\,8313 and UGC\,8365, and a gas cloud candidate which almost connects to the main disk. The cloud candidate and UGC\,8365 follow the velocity orientation of the disk, although the velocity difference between NGC\,5055 and UGC\,8365 is so large that it is doubtful they are in the same dynamical system. UGC\,8313's systemic velocity is such that it coincides with the velocities in the receding side of NGC\,5055 while its location is on the approaching side. 
\subsubsection{NGC 5585} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_n5585.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the NGC\,5585 field overlaid on a KPNO $R$-band image.} 
\label{fig:Overview_n5585.pdf}
\end{figure*}
This galaxy is a spiral galaxy with an \hi\ disk that extends significantly beyond the optical detection in the DSS image and that is slightly warped. Besides the target, we detect a single cloud candidate at a projected distance of 58 kpc. The cloud candidate shows a hint of a velocity structure but as it is barely resolved this could be an artifact of the masking. If this cloud is part of the dynamical system describing NGC\,5585 it would be counter rotating. 
\subsubsection{UGC 4278} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_u4278.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the UGC\,4278 field.} 
\label{fig:Overview_u4278.pdf}
\end{figure*}
Besides the target galaxy we find one other source in the field that we deem to be real, the companion NGC\,2537. We do not detect anything in between the two sources and their disks appear regular. This leads us to believe that there is currently no interaction between the galaxies. If they were dynamically connected their velocity structure is such that NGC\,2537 would be counter rotating in the frame of UGC\,4278 but in the frame of NGC\,2357 the target would be co-rotating. 
\subsubsection{UGC 7774} 
\begin{figure*}[htbp] 
\centering 
\includegraphics[width = 18 cm]{Figures_App_New/Overview_u7774.pdf} 
\caption{As Figure \ref{fig:Overview_n0925.pdf} but for the UGC\,7774 field overlaid on a DSS 2 $R$-band image.} 
\label{fig:Overview_u7774.pdf}
\end{figure*}
UGC\,7774 is an edge-on galaxy with one of the most striking examples of a warp known (see Figure \ref{fig:Overview_u7774.pdf}). We detect a single companion at a rather large distance from the galaxy (d$_{\rm proj} \sim$ 232 kpc). This companion does appear quite disturbed and hence it might be related to UGC\,7774's warp however a detailed analysis would be required to further this idea. Its systemic velocity is aligned with the  rotation in the western side of UGC\,7774.\\ 


==> Target_Table.tex <==
% This file contains the table with cloud host galaxy info. 
\begin{table*}[h!] 
\caption{Properties of the galaxies in the HALOGAS sample.} \label{table:hosts} 
\centering  
\begin{tabular}{l l l l l l l l l l l l l l} 
\hline 
Galaxy & Dist. & $\rm{ v_{sys}}$ & W$_{20}$ & R$_{\rm max}$ & R$_{\rm min}$& M$_*$ &  M$_{HI}$ & M$_{\rm dyn}$  &r$_{\rm vir}$\tablefootmark{d} & SFR\tablefootmark{e} & $\tau$ & D$_{25}$ & $i$  \\ 
        &  Mpc &  \kms  &  \kms  & kpc & kpc & $10^{9}$\,\msun & $10^{8}$\,\msun & $10^{10}$\,\msun &kpc  & \msun yr$^{-1}$ & $10^9\,yr$ & kpc & $^{\circ}$  \\ 
\hline 
NGC\,0925  &        9.1 &      550.8&      222.0 &       28.1 &       19.8 &       7.48 \tablefootmark{a),b),c)  } &      54.6 &       12.3 &      103.0 &       0.77 &        7.1 &       29.9 & 54\\
NGC\,0949  &       11.3 &      607.7&      207.2 &       13.3 &        6.0 &       3.43 \tablefootmark{c)        } &       5.6 &        5.3 &       78.0 &       0.31 &        1.8 &       11.5 & 52\\
NGC\,1003  &       11.6 &      621.2&      229.6 &       35.8 &        7.4 &       3.04 \tablefootmark{c)        } &      59.3 &       12.9 &      104.7 &       0.40 &       14.8 &       21.3 & 67\\
NGC\,2541  &       12.0 &      555.1&      209.4 &       28.3 &       12.5 &       1.65 \tablefootmark{c)        } &      47.5 &        8.5 &       91.0 &       0.35 &       13.6 &       25.1 & 67\\
NGC\,3198  &       14.5 &      659.6&      317.4 &       48.1 &       12.9 &      22.13 \tablefootmark{a),b),c)  } &     112.4 &       31.5 &      140.9 &       1.10 &       10.2 &       37.1 & 71\\
NGC\,4062  &       16.9 &      767.7&      310.8 &       18.0 &        7.2 &       0.11 \tablefootmark{c)        } &      17.5 &       11.7 &      101.4 &       0.67 &        2.6 &       22.1 & 68\\
NGC\,4244  &        4.4 &      245.8&      216.3 &       17.7 &        3.7 &       2.33 \tablefootmark{a),b),c)  } &      18.0 &        4.8 &       75.3 &       0.12 &       15.0 &       20.2 & 90\\
NGC\,4258  &        7.6 &      444.6&      435.8 &       28.9 &       12.4 &      65.88 \tablefootmark{b),c)     } &      57.1 &       35.6 &      146.8 &       1.70 &        3.4 &       37.8 & 71\\
NGC\,4274  &       19.4 &      933.0&      463.0 &       19.6 &        7.2 &      71.94 \tablefootmark{c)        } &       7.9 &       27.0 &      133.8 &       1.20 &        0.7 &       36.7 & 72\\
NGC\,4414  &       17.8 &      718.6&      395.6 &       37.5 &       26.0 &      65.55 \tablefootmark{c)        } &      50.1 &       58.2 &      172.8 &       4.20 &        1.2 &       23.3 & 50\\
NGC\,4448  &        9.7\tablefootmark{f} &      647.5&      382.8 &        4.4 &        2.4 &      8.760 \tablefootmark{c)        } &       0.4 &        4.2 &       71.8 &       0.06 &        0.8 &       10.7 & 71\\
NGC\,4559  &        7.9 &      809.6&      253.1 &       21.8 &        9.1 &       6.32 \tablefootmark{a),b),c)  } &      43.6 &        9.3 &       93.9 &       0.69 &        6.3 &       26.0 & 69\\
NGC\,4565  &       10.8 &     1237.8&      517.4 &       34.7 &        6.0 &      71.18 \tablefootmark{a),b),c)  } &      69.8 &       54.0 &      168.6 &       0.67 &       10.4 &       50.9 & 90\\
NGC\,5023  &        6.6 &      405.9&      192.2 &        9.8 &        2.5 &       1.51 \tablefootmark{a),b),c)  } &       5.8 &        2.1 &       57.2 &       0.04 &       14.8 &       13.1 & 90\\
NGC\,5055  &        8.5 &      498.1&      393.5 &       45.4 &       27.8 &      69.03 \tablefootmark{a),b),c)  } &      73.5 &       60.9 &      175.5 &       2.10 &        3.5 &       32.1 & 55\\
NGC\,5229  &        5.1 &      356.9&      138.9 &        5.1 &        1.6 &      0.004 \tablefootmark{c)        } &       1.4 &        0.6 &       37.1 &       0.01 &       16.8 &        5.2 & 90\\
NGC\,5585  &        8.7 &      306.9&      161.7 &       19.6 &       15.2 &       1.49 \tablefootmark{c)        } &      26.1 &        4.9 &       76.0 &       0.41 &        6.4 &       13.9 & 51\\
UGC\,2082  &       14.1 &      706.4&      208.0 &       23.6 &        5.8 &       2.40 \tablefootmark{c)        } &      23.4 &        5.9 &       80.8 &       0.04 &       57.0 &       23.8 & 89\\
UGC\,4278  &       13.6 &      559.6&      192.7 &       13.5 &        5.3 &       1.50 \tablefootmark{a),b),c)  } &      20.0 &        2.9 &       63.8 &       0.18 &       11.1 &       17.0 & 90\\
UGC\,7774  &       24.4 &      521.7&      205.5 &       33.6 &        9.0 &        nan \tablefootmark{          } &      35.4 &        8.3 &       90.2 &       0.10 &       37.3 &       24.8 & 90\\
\hline 
\end{tabular} 
\tablefoot{  
\tablefoottext{a}{Galaxy integrated flux  taken from \cite{Clark2018}, mass calculated using 3.6 and 4.5 $\mu$m following \cite{Eskew2012}.}  
\tablefoottext{b}{Galaxy integrated flux taken from \cite{Clark2018},  calculated using 3.4 and 4.6 $\mu$m following \cite{Cluver2014}.}  
\tablefoottext{c}{Galaxy integrated flux taken from \cite{Skrutskie2006},  mass calculated using 3.6 $\mu$m following \cite{McGaugh2014}.}  
\tablefoottext{d}{Derived from dynamical mass.}  
\tablefoottext{e}{SFR from the pilot paper.}  
\tablefoottext{f}{This distance is likely an underestimate by a factor of two.}  
} 
 \end{table*}  


==> Threshold_Table.tex <==
% This file contains the final thresholding table 
\begin{table} 
\caption{Noise cut limits and beam sizes used in \sofia for each data cube.} \label{table:cuts} 
\centering  
\begin{tabular}{lcl} 
\hline 
Data cube & Int. SNR Threshold & FWHM$_{maj}\times$FWHM$_{min}$ \\ 
\hline 
NGC\,0672 & 32.5 & 31.6"$\times$14.3" \\ 
NGC\,0925 & 30.5 & 26.6"$\times$14.9" \\ 
NGC\,0949 & 28.9 & 24.2"$\times$14.7" \\ 
NGC\,1003 & 27.9 & 22.6"$\times$14.7" \\ 
NGC\,2541 & 26.3 & 19.1"$\times$15.4" \\ 
NGC\,3198 & 26.9 & 21.0"$\times$14.8" \\ 
NGC\,4062 & 30.9 & 27.6"$\times$14.8" \\ 
NGC\,4244 & 29.2 & 23.9"$\times$15.2" \\ 
NGC\,4258 & 26.9 & 20.9"$\times$14.7" \\ 
NGC\,4274 & 31.7 & 29.5"$\times$14.5" \\ 
NGC\,4414 & 31.7 & 28.6"$\times$15.0" \\ 
NGC\,4448 & 32.1 & 30.5"$\times$14.4" \\ 
NGC\,4559 & 32.4 & 31.2"$\times$14.3" \\ 
NGC\,4565 & 34.1 & 33.5"$\times$14.8" \\ 
NGC\,4631 & 31.6 & 27.8"$\times$15.3" \\ 
NGC\,5023 & 27.1 & 21.3"$\times$14.7" \\ 
NGC\,5055 & 27.4 & 22.1"$\times$14.5" \\ 
NGC\,5229 & 26.8 & 20.1"$\times$15.2" \\ 
NGC\,5585 & 24.9 & 17.5"$\times$15.0" \\ 
UGC\,2082 & 32.0 & 31.8"$\times$13.8" \\ 
UGC\,4278 & 26.9 & 20.7"$\times$14.9" \\ 
UGC\,7774 & 28.4 & 23.3"$\times$14.8" \\ 
\hline 
\end{tabular} 
\end{table} 


==> sources_Table.tex <==
% This file contains the final sources table 
\onecolumn
\begin{landscape}\begin{longtable}{lllllllllllll}
\caption{\sofia\ detected sources.} \label{table:detec}\\ 
\hline 
Galaxy & ID & RA & Dec & Class & S$_{p}$ & $F_{i}$ & $F_{i}$,pbcorr& W20  & Vel. & Dist. to target & Flag & Counterpart \\ 
  &   &  [hms] & [dms] & & [mJy  bm$^{-1}$] & [Jy \kms]  & [Jy \kms]& [\kms] & [\kms] & [kpc] &  & \\ 
   (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13)  \\  
\hline 
\endfirsthead 
\caption{continued.}\\ 
\hline 
Galaxy & ID & RA & Dec & Class  & S$_{p}$ & $F_{i}$ & $F_{i}$-pbcorr& W20  & Vel. & Dist. to target & Flag & Counterpart  \\ 
  &   &  [hms] & [dms] & &  [mJy bm$^{-1}$] & [Jy \kms] & [Jy \kms] & [\kms] & [\kms] & [kpc] &  &  \\ 
   (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13)  \\  
\hline 
\endhead 
\hline 
\endfoot 
 
NGC\,0672 \tablefootmark{a} & 1          & 1h47m46.75s  & 27d24m9.62s  & T      & 53.474     & 249.158    & 252.323   & 276.9      & 397.1      & 0.0        & 1     & NGC\,672+IC\,1727              \\ 
NGC\,0672  & 7          & 1h46m22.55s  & 27d44m7.89s  & A      & 0.998      & 0.057      & 0.298     & 43.7       & 357.9      & 60.4       & 4     &                                \\ 
NGC\,0925 \tablefootmark{a} & 1          & 2h27m14.86s  & 33d34m53.99s & T      & 36.194     & 279.347    & 279.462   & 222.0      & 550.8      & 0.0        & 1     & NGC\,925                       \\ 
NGC\,0925  & 4          & 2h27m19.97s  & 33d57m30.11s & C      & 2.963      & 0.196      & 0.599     & 35.5       & 641.8      & 59.9       & 1     & Halogas                        \\ 
NGC\,0949 \tablefootmark{a} & 1          & 2h30m49.08s  & 37d8m18.34s  & T      & 13.686     & 18.522     & 18.522    & 207.2      & 607.7      & 0.0        & 1     & NGC\,949                       \\ 
NGC\,0949  & 2          & 2h28m1.99s   & 37d3m38.76s  & A      & 1.165      & 0.089      & 1.252     & 534.4      & 848.4      & 110.6      & 4     & Bad\,continuum\,subtraction.   \\ 
NGC\,1003 \tablefootmark{a} & 1          & 2h39m17.82s  & 40d52m20.74s & T      & 36.422     & 186.582    & 186.594   & 229.6      & 621.2      & 0.0        & 1     & NGC\,1003                      \\ 
NGC\,2541  & 1          & 8h12m39.68s  & 48d36m41.05s & C      & 1.369      & 0.096      & 1.347     & 47.0       & 517.4      & 117.0      & 1     & WISEA\,J081239.49+483645.3     \\ 
NGC\,2541 \tablefootmark{a} & 2          & 8h14m39.75s  & 49d3m46.30s  & T      & 29.115     & 139.790    & 139.793   & 209.4      & 555.1      & 0.0        & 1     & NGC\,2541                      \\ 
NGC\,3198 \tablefootmark{a} & 1          & 10h19m55.03s & 45d32m55.04s & T      & 24.100     & 226.582    & 226.586   & 317.4      & 659.6      & 0.0        & 1     & NGC\,3198                      \\ 
NGC\,3198  & 2          & 10h18m43.05s & 46d2m55.56s  & C      & 2.486      & 0.463      & 5.322     & 76.8       & 584.9      & 137.2      & 1     & VV\,834\,NED02                 \\ 
NGC\,4062 \tablefootmark{a} & 1          & 12h4m4.04s   & 31d53m43.28s & T      & 17.084     & 25.936     & 25.936    & 310.8      & 767.7      & 0.0        & 1     & NGC\,4062                      \\ 
NGC\,4244 \tablefootmark{a} & 1          & 12h17m28.97s & 37d48m20.46s & T      & 83.074     & 393.036    & 393.079   & 216.3      & 245.8      & 0.0        & 1     & NGC\,4244                      \\ 
NGC\,4244  & 2          & 12h18m41.54s & 37d41m40.03s & A      & 0.724      & 0.299      & 0.501     & 64.1       & 176.2      & 20.3       & 4     &                                \\ 
NGC\,4244  & 3          & 12h17m8.30s  & 38d1m27.46s  & A      & 1.095      & 1.384      & 2.038     & 62.2       & 170.4      & 17.6       & 4     &                                \\ 
NGC\,4244  & 4          & 12h16m43.51s & 37d46m18.88s & A      & 1.023      & 0.069      & 0.083     & 41.6       & 224.6      & 11.8       & 4     &                                \\ 
NGC\,4244  & 5          & 12h16m31.94s & 37d53m54.14s & A      & 0.953      & 3.781      & 5.265     & 77.0       & 308.9      & 16.1       & 4     &                                \\ 
NGC\,4244  & 6          & 12h17m50.07s & 38d4m58.72s  & A      & 0.603      & 0.055      & 0.100     & 46.7       & 265.3      & 22.0       & 4     &                                \\ 
NGC\,4244  & 7          & 12h18m3.79s  & 37d35m3.38s  & A      & 0.937      & 0.489      & 0.781     & 69.5       & 324.4      & 19.2       & 4     &                                \\ 
NGC\,4244  & 8          & 12h18m9.03s  & 37d40m6.91s  & A      & 0.927      & 0.582      & 0.760     & 52.9       & 328.3      & 14.6       & 4     &                                \\ 
NGC\,4258 \tablefootmark{a} & 1          & 12h18m55.27s & 47d17m52.04s & T      & 36.034     & 418.909    & 419.152   & 435.8      & 444.6      & 0.0        & 1     & MESSIER\,106                   \\ 
NGC\,4258  & 4          & 12h18m11.10s & 46d55m3.52s  & C      & 5.577      & 0.851      & 3.148     & 79.0       & 397.4      & 53.1       & 1     & SDSS\,J121811.04+465501.2      \\ 
NGC\,4258  & 5          & 12h18m56.49s & 47d5m22.48s  & A      & 1.041      & 0.133      & 0.187     & 35.9       & 441.0      & 27.6       & 3     &                                \\ 
NGC\,4258  & 6          & 12h17m50.73s & 47d24m25.38s & C      & 8.142      & 1.922      & 2.709     & 84.9       & 483.5      & 28.2       & 1     & NGC\,4248                      \\ 
NGC\,4258  & 7          & 12h18m13.34s & 47d13m21.86s & A      & 0.873      & 0.090      & 0.106     & 37.7       & 514.0      & 18.6       & 4     &                                \\ 
NGC\,4258  & 9          & 12h15m53.26s & 47d5m51.19s  & C      & 2.020      & 1.668      & 23.763    & 388.4      & 976.9      & 73.3       & 1     & NGC\,4217                      \\ 
NGC\,4258  & 10         & 12h19m27.48s & 47d18m42.60s & C*     & 1.811      & 0.057      & 0.060     & 39.0       & 811.3      & 12.2       & 1     & WISEA\,J121927.11+471844.3     \\ 
NGC\,4258  & 11         & 12h19m33.39s & 47d27m1.63s  & C      & 1.329      & 0.037      & 0.046     & 29.5       & 941.1      & 24.8       & 1     & WISEA\,J121933.24+472705.1     \\ 
NGC\,4274  & 1          & 12h20m9.23s  & 29d16m39.95s & C      & 1.011      & 2.319      & 5.725     & 472.3      & 637.8      & 117.1      & 1     & NGC\,4278                      \\ 
NGC\,4274  & 6          & 12h20m42.02s & 29d20m47.03s & C      & 1.969      & 0.384      & 0.865     & 128.6      & 644.1      & 111.7      & 1     & NGC\,4286                      \\ 
NGC\,4274 \tablefootmark{a} & 8          & 12h19m49.73s & 29d36m58.74s & T      & 7.013      & 8.883      & 8.884     & 463.0      & 933.0      & 0.0        & 1     & NGC\,4274                      \\ 
NGC\,4414 \tablefootmark{a} & 1          & 12h26m26.47s & 31d13m4.40s  & T      & 19.786     & 66.938     & 66.956    & 395.6      & 718.6      & 0.0        & 1     & NGC\,4414                      \\ 
NGC\,4414  & 7          & 12h24m13.24s & 31d31m9.96s  & C      & 2.333      & 1.629      & 23.095    & 196.8      & 1226.5     & 174.5      & 1     & NGC\,4359                      \\ 
NGC\,4448 \tablefootmark{a} & 1          & 12h28m15.33s & 28d37m13.98s & T      & 4.307      & 1.917      & 1.917     & 382.8      & 647.5      & 0.0        & 1     & NGC\,4448                      \\ 
NGC\,4448  & 2          & 12h26m9.77s  & 28d27m57.87s & C      & 1.769      & 0.236      & 1.577     & 53.3       & 1213.6     & 82.1       & 1     & IC\,3334                       \\ 
NGC\,4559 \tablefootmark{a} & 1          & 12h35m58.54s & 27d57m31.09s & T      & 41.176     & 296.186    & 296.216   & 253.1      & 809.6      & 0.0        & 1     & NGC\,4559                      \\ 
NGC\,4559  & 2          & 12h35m21.34s & 27d33m44.64s & C      & 2.300      & 0.143      & 0.570     & 50.3       & 1201.9     & 57.8       & 1     & WISEA\,J123521.10+273342.9     \\ 
NGC\,4565  & 1          & 12h37m1.18s  & 26d2m8.30s   & C*     & 2.790      & 0.078      & 0.093     & 25.7       & 856.2      & 30.7       & 1     & SDSS\,J123701.22+260208.5      \\ 
NGC\,4565 \tablefootmark{a} & 2          & 12h36m19.01s & 25d59m43.72s & T      & 63.489     & 253.191    & 253.430   & 517.4      & 1237.8     & 0.0        & 1     & HIJASS\,J1236+25               \\ 
NGC\,4565  & 4          & 12h35m34.84s & 25d51m3.95s  & C      & 10.837     & 4.418      & 6.326     & 140.7      & 1345.2     & 41.4       & 1     & NGC\,4562                      \\ 
NGC\,4565  & 5          & 12h36m20.09s & 26d5m1.24s   & C      & 10.387     & 1.337      & 1.431     & 43.9       & 1262.2     & 16.6       & 1     & IC\,3571                       \\ 
NGC\,4631 \tablefootmark{a} & 1          & 12h42m7.55s  & 32d32m14.76s & T      & 74.905     & 614.285    & 614.367   & 319.0      & 602.6      & 0.1        & 1     & NGC\,4631                      \\ 
NGC\,4631  & 2          & 12h43m55.95s & 32d10m28.93s & C      & 4.939      & 41.146     & 415.921   & 200.3      & 640.6      & 69.9       & 1     & 2MASS\,J12435666+3210138       \\ 
NGC\,4631  & 3          & 12h43m39.49s & 32d33m2.54s  & A      & 1.762      & 4.448      & 9.770     & 44.0       & 644.9      & 43.0       & 4     &                                \\ 
NGC\,4631  & 6          & 12h41m47.46s & 32d51m11.44s & A+C    & 5.648      & 1.089      & 2.373     & 60.2       & 682.3      & 42.9       & 2     & SDSS\,J124146.99+325124.8      \\ 
NGC\,4631  & 7          & 12h43m59.45s & 32d31m49.21s & A      & 1.189      & 0.083      & 0.274     & 47.9       & 681.2      & 52.2       & 4     &                                \\ 
NGC\,4631  & 8          & 12h41m26.89s & 32d20m51.36s & A      & 1.357      & 0.286      & 0.442     & 37.3       & 705.9      & 31.5       & 4     &                                \\ 
NGC\,4631  & 9          & 12h40m9.81s  & 32d39m20.10s & C      & 5.240      & 1.114      & 4.811     & 85.9       & 765.2      & 56.9       & 1     & SDSS\,J124010.08+323930.4      \\ 
NGC\,4631  & 10         & 12h43m7.01s  & 32d29m27.92s & C      & 7.686      & 0.929      & 1.302     & 66.3       & 899.6      & 28.5       & 1     & MCG\,+06-28-022                \\ 
NGC\,4631  & 11         & 12h42m1.52s  & 32d24m4.83s  & C*     & 2.377      & 0.082      & 0.095     & 35.1       & 908.3      & 18.2       & 1     & SDSS\,J124201.68+322356.8      \\ 
NGC\,5023 \tablefootmark{a} & 1          & 13h12m11.73s & 44d2m18.91s  & T      & 40.568     & 56.017     & 56.022    & 192.2      & 405.9      & 0.0        & 1     & NGC\,5023                      \\ 
NGC\,5055 \tablefootmark{a} & 1          & 13h15m45.64s & 42d1m26.13s  & T      & 22.779     & 430.681    & 431.171   & 393.5      & 498.1      & 0.0        & 1     & MESSIER\,63                    \\ 
NGC\,5055  & 4          & 13h13m54.32s & 42d12m39.61s & C      & 5.069      & 1.474      & 5.117     & 123.4      & 619.5      & 58.1       & 1     & UGC\,8313                      \\ 
NGC\,5055  & 6          & 13h18m44.29s & 41d56m57.63s & C      & 1.479      & 0.551      & 6.761     & 137.6      & 1265.3     & 82.8       & 1     & UGC\,8365                      \\ 
NGC\,5229 \tablefootmark{a} & 1          & 13h34m3.22s  & 47d54m49.51s & T      & 31.071     & 23.533     & 23.534    & 138.9      & 356.9      & 0.0        & 1     & NGC\,5229                      \\ 
NGC\,5585 \tablefootmark{a} & 2          & 14h19m49.28s & 56d44m1.81s  & T      & 24.749     & 146.362    & 146.392   & 161.7      & 306.9      & 0.0        & 1     & NGC\,5585                      \\ 
UGC\,2082 \tablefootmark{a} & 1          & 2h36m15.97s  & 25d25m25.56s & T      & 43.440     & 49.840     & 49.841    & 208.0      & 706.4      & 0.0        & 1     & UGC\,2082                      \\ 
UGC\,4278  & 1          & 8h14m30.44s  & 45d56m42.79s & A      & 1.958      & 0.127      & 0.183     & 179.9      & -124.8     & 52.5       & 4     &                                \\ 
UGC\,4278  & 2          & 8h14m30.45s  & 45d56m43.22s & A      & 1.791      & 0.070      & 0.101     & 77.2       & 64.2       & 52.5       & 4     &                                \\ 
UGC\,4278  & 3          & 8h14m30.49s  & 45d56m43.28s & A      & 1.822      & 0.143      & 0.206     & 197.6      & 194.1      & 52.5       & 4     &                                \\ 
UGC\,4278  & 4          & 8h13m14.79s  & 45d59m22.38s & C      & 6.853      & 12.274     & 21.774    & 113.2      & 448.9      & 65.6       & 1     & NGC\,2537                      \\ 
UGC\,4278 \tablefootmark{a} & 6          & 8h13m58.62s  & 45d44m39.78s & T      & 57.354     & 45.789     & 45.789    & 192.7      & 559.6      & 0.0        & 1     & IC\,2233                       \\ 
UGC\,4278  & 7          & 8h12m42.27s  & 45d36m54.45s & A      & 1.218      & 0.092      & 0.151     & 311.8      & 914.8      & 61.0       & 4     &                                \\ 
UGC\,4278  & 8          & 8h14m30.47s  & 45d56m42.78s & A      & 2.645      & 0.159      & 0.228     & 130.7      & 1319.9     & 52.5       & 4     &                                \\ 
UGC\,7774 \tablefootmark{a} & 1          & 12h36m23.16s & 40d0m18.06s  & T      & 31.820     & 25.198     & 25.198    & 205.5      & 521.7      & 0.0        & 1     & UGC\,7774                      \\ 
UGC\,7774  & 2          & 12h33m53.14s & 39d37m28.21s & C      & 1.177      & 0.220      & 5.888     & 40.8       & 654.9      & 260.9      & 1     & MCG\,+07-26-024                \\ 
\end{longtable} 
 \tablefoot{ 
\tablefoottext{*}{These cloud candidates have a counterpart identification that can not be confirmed in velocity.} 
\tablefoottext{a}{These are the values for the cloud searching \sofia\ run performed in this study.} 
} 
\end{landscape}
\twocolumn 

